A Note on Output Length of One-Way State Generators and EFIs

We study the output length of one-way state generators (OWSGs), their weaker variants, and EFIs. - Standard OWSGs. Recently, Cavalar et al. (arXiv:2312.08363) give OWSGs with $m$-qubit outputs for any $m=\omega(\log \lambda)$, where $\lambda$ is the security parameter, and conjecture that there do not exist OWSGs with $O(\log \log \lambda)$-qubit outputs. We prove their conjecture in a stronger manner by showing that there do not exist OWSGs with $O(\log \lambda)$-qubit outputs. This means that their construction is optimal in terms of output length. - Inverse-polynomial-advantage OWSGs. Let $\epsilon$-OWSGs be a parameterized variant of OWSGs where a quantum polynomial-time adversary's advantage is at most $\epsilon$. For any constant $c\in \mathbb{N}$, we construct $\lambda^{-c}$-OWSGs with $((c+1)\log \lambda+O(1))$-qubit outputs assuming the existence of OWFs. We show that this is almost tight by proving that there do not exist $\lambda^{-c}$-OWSGs with at most $(c\log \lambda-2)$-qubit outputs. - Constant-advantage OWSGs. For any constant $\epsilon>0$, we construct $\epsilon$-OWSGs with $O(\log \log \lambda)$-qubit outputs assuming the existence of subexponentially secure OWFs. We show that this is almost tight by proving that there do not exist $O(1)$-OWSGs with $((\log \log \lambda)/2+O(1))$-qubit outputs. - Weak OWSGs. We refer to $(1-1/\mathsf{poly}(\lambda))$-OWSGs as weak OWSGs. We construct weak OWSGs with $m$-qubit outputs for any $m=\omega(1)$ assuming the existence of exponentially secure OWFs with linear expansion. We show that this is tight by proving that there do not exist weak OWSGs with $O(1)$-qubit outputs. - EFIs. We show that there do not exist $O(\log \lambda)$-qubit EFIs. We show that this is tight by proving that there exist $\omega(\log \lambda)$-qubit EFIs assuming the existence of exponentially secure PRGs.

==> EFI_old.tex <==
\section{Output Length of EFI Pairs}
\label{sec:EFI}
Here we show a lowerbound for the output length of EFI pairs.
\begin{theorem}
There do not exist EFI pairs with $O(\log\secp)$-qubit outputs.
\end{theorem}

\begin{proof}
Let $(\rho_0,\rho_1)$ be an EFI pair. For each $b\in\bit$, let $m$ be the number of qubits of $\rho_b$,
and let $\rho_b=\sum_i p_{b,i}|\phi_{b,i}\rangle\langle\phi_{b,i}|$    
be $\rho_b$'s diagonalization.
Then,
\begin{align}
1-\negl(\secp)&\le \|\rho_0-\rho_1\|_{tr}    \\
&=
\left\|\sum_{i}p_{0,i}|\phi_{0,i}\rangle\langle\phi_{0,i}|-\sum_{j}p_{1,j}|\phi_{1,j}\rangle\langle\phi_{1,j}|\right\|_{tr}\\
&=\left\|\sum_{i,j}p_{0,i}p_{1,j}\left(|\phi_{0,i}\rangle\langle\phi_{0,i}|-|\phi_{1,j}\rangle\langle\phi_{1,j}|\right)\right\|_{tr}\\
&\le \sum_{i,j}p_{0,i}p_{1,j}\left\||\phi_{0,i}\rangle\langle\phi_{0,i}|-|\phi_{1,j}\rangle\langle\phi_{1,j}|\right\|_{tr}\\ 
&= \sum_{i,j}p_{0,i}p_{1,j}\sqrt{1-|\langle \phi_{0,i}|\phi_{1,j}\rangle|^2}\\
&\le  \sqrt{1-\sum_{i,j}p_{0,i}p_{1,j}|\langle \phi_{0,i}|\phi_{1,j}\rangle|^2}\\
&\le  \sqrt{1-\frac{1}{4}\sum_{b,b'}\sum_{i,j}p_{b,i}p_{b',j}|\langle \phi_{b,i}|\phi_{b',j}\rangle|^2+\negl(\secp)}\label{swaptest}\\
&\le \sqrt{1-2^{-m}+\negl(\secp)}, 
\end{align}
which is a contradiction if $m=O(\log\secp)$,
and therefore the theorem is shown.
Here, \cref{swaptest} is derived as follows.
First, from the straightforward calculation,
\begin{align}
   \sum_{b,b'}\sum_{i,j}p_{b,i}p_{b',j}|\langle\phi_{b,i}|\phi_{b',j}\rangle|^2 
   =\sum_ip_{0,i}^2+\sum_ip_{1,i}^2
   +2\sum_{i,j}p_{0,i}p_{1,j}|\langle\phi_{0,i}|\phi_{1,j}\rangle|^2.\label{swap1}
\end{align}
Second, we have
\begin{align}
\left|\sum_ip_{b,i}^2- \sum_{i,j}p_{0,i}p_{1,j}|\langle\phi_{0,i}|\phi_{1,j}\rangle|^2\right|\le\negl(\secp)    \label{swap2}
\end{align}
for each $b\in\bit$, because otherwise the QPT adversary who does the swap test 
can distinguish $\rho_0$ and $\rho_1$.\footnote{Consider the following QPT adversary: given $\rho_b$, run the swap test between
it and $\rho_0$. The probability that the adversary accepts is $p_b\coloneqq\frac{1+\Tr(\rho_b\rho_0)}{2}$. Due to the computational
indistinguishability of $\rho_0$ and $\rho_1$, $|p_0-p_1|\le\negl(\secp)$, which means that
$|\Tr(\rho_0^2)-\Tr(\rho_0\rho_1)|\le\negl(\secp)$.}
By combining \cref{swap1} and \cref{swap2},
we can derive 
\cref{swaptest}.
\end{proof}

==> complexity.tex <==
\subsection{Complexity Theoretic Barries} 
\begin{theorem}
If there exist weak OWSGs with $O(\log\log \secp)$-qubit outputs,  $\mathbf{QCMA}$ is average-case subexponential quantum hard. \takashi{need to make it more formal.}
\end{theorem}

==> succinct_comm.tex <==
\section{Commitment Length of Quantum Bit Commitments}
\label{sec:succinct_comm}

\subsection{Preliminaries}
\begin{definition}[Non-Interactive Quantum Bit Commitments~\cite{AC:Yan22}]
A non-interactive quantum bit commitment scheme is   
a family $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in{\mathbb N}}$ of efficiently implementable unitary operators that is used as follows.
\begin{itemize}
    \item[{\bf Commit phase:}]
    In the commit phase, the sender who wants to commit $b\in\bit$ generates the state
    $\ket{\Psi_b}_{\regR,\regC}\coloneqq Q_b(\secp)|0...0\rangle$ over two registers $\regR$ and $\regC$.
    The sender sends the commitment register $\regC$ to the receiver.
    \item[{\bf Reveal phase:}]
    In the reveal phase, the sender sends the reveal register $\regR$ and $b$ to the receiver.
    The receiver applies $Q_b^\dagger(\secp)$ on the state over $\regR$ and $\regC$,
    and measures all qubits in the computational basis. If all results are 0,
    the receiver accepts $b$.
    Otherwise, the receiver rejects.
\end{itemize}
\end{definition}
For the notational simplicity, we often omit the security parameter $\secp$ of $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in{\mathbb N}}$,
and just write as $(Q_0,Q_1)$.

\begin{definition}[Hiding]
We say that a commitment scheme $(Q_0,Q_1)$ is statistically (resp. computationally) hiding if    
\begin{align}
|\Pr[1\gets\cA(1^\secp,\rho_0)]    
-\Pr[1\gets\cA(1^\secp,\rho_1)]|\le\negl(\secp)    
\end{align}
for any unbounded (resp. QPT) adversary $\cA$, where
$\rho_b\coloneqq \Tr_{\regR}(\ket{\Psi_b}_{\regR,\regC})$,
and $\Tr_{\regA}(\sigma_{\regA,\regB})$
means tracing out the register $\regA$ of the state $\sigma_{\regA,\regB}$ over two registers $\regA$ and $\regB$.
\end{definition}

\begin{definition}[Binding]
\label{def:honest_binding}
We say that a commitment scheme $(Q_0,Q_1)$ is statistically (resp. computationally) binding if    
the winning probability of the following security game is $\negl(\secp)$ for any unbounded (resp. QPT) adversary $\cA$.
\begin{enumerate}
    \item 
    $\cA$ (who plays the role of the sender) honestly commits 0.
    \item 
    $\cA$ applies any operation on the register $\regR$.
    \item 
    $\cA$ opens the commitment to 1. 
    \item 
    $\cA$ wins
    if and only if the receiver accepts 1.
\end{enumerate}
\end{definition}
\begin{remark}
The above definition of binding, so-called honest binding, does not capture all possible attacks,
because we assume that the adversary honestly commits 0 in the commit phase.
However, when we want to show lower bounds, restricting to the honest binding only strengthens our results, because any reasonable definition of binding should satisfy the honest binding.
Moreover, it is shown in \cite{AC:Yan22} that the honest binding implies a standard definition of binding, so-called sum-binding~\cite{EC:DumMaySal00}, which captures general attacks. 
In the following, if we just say binding, it means honest binding.
\end{remark}

\begin{lemma}[Flavor Conversion~\cite{EC:HhaMorYam23}]
\label{lem:flavor}
Let $(Q_0,Q_1)$ be a statistically-hiding (resp. binding) and computationally-binding (resp. hiding) non-interactive quantum bit commitment scheme.
Then, $(\tilde{Q}_0,\tilde{Q}_1)$ defined as follows is
a statistically-binding (resp. hiding) and computationally-hiding (resp. binding) non-interactive quantum bit commitment scheme.
\begin{align}
\ket{\tilde{\Psi}_b}_{\regR',\regC'}\coloneqq 
\tilde{Q}_b|0...0\rangle\coloneqq
\frac{1}{\sqrt{2}}\left[
|0\rangle_\regD \otimes(Q_0|0...0\rangle)_{\regR,\regC} 
+ (-1)^b|1\rangle_\regD \otimes(Q_1|0...0\rangle)_{\regR,\regC}   
\right]
\end{align}
for each $b\in\bit$,
where $\regR'\coloneqq \regC$
and $\regC'\coloneqq (\regR,\regD)$.
\end{lemma}

\begin{lemma}\label{lem:TrF}
For any two states $\rho$ and $\sigma$, $\Tr(\rho\sigma)\le F(\rho,\sigma)$,    
where $F$ is the fidelity.
\end{lemma}

\begin{proof}[Proof of \cref{lem:TrF}]
The operator $\sqrt{\sigma}\rho\sqrt{\sigma}$ is positive semi-definite.    
Therefore, it has the diagonalization $\sqrt{\sigma}\rho\sqrt{\sigma}=\sum_i \alpha_i |\phi_i\rangle\langle \phi_i|$,
where $\alpha_i\ge0$ for all $i$.
Hence
\begin{align}
F(\rho,\sigma)=\left(\Tr\sqrt{\sqrt{\sigma}\rho\sqrt{\sigma}}\right)^2    
=\left(\sum_i\sqrt{\alpha_i}\right)^2    
=\sum_i\alpha_i+\sum_{i\neq j}\sqrt{\alpha_i\alpha_j}    
\ge\sum_i\alpha_i
=\Tr(\rho\sigma).
\end{align}
\end{proof}


\begin{lemma}
\label{lem:fidelity_upperbound} 
Let $\{\ket{\psi_k}\}_{k\in \bit^n}$ be any set of pure states.
Then
\begin{align}
F\left(\frac{1}{2^n}\sum_{k\in\bit^n}\ket{\psi_k}\bra{\psi_k},\frac{I^{\otimes m}}{2^m}\right)
\le \frac{2^n}{2^m}.
\end{align}
\end{lemma}

\begin{proof}
Let $\sum_{k\in\bit^n}\alpha_k\ket{\phi_k}\bra{\phi_k}$ be a diagonalization of
$\frac{1}{2^n}\sum_{k\in\bit^n}\ket{\psi_k}\bra{\psi_k}$.
Then
\begin{align}
F\left(\frac{1}{2^n}\sum_{k\in\bit^n}\ket{\psi_k}\bra{\psi_k},\frac{I^{\otimes m}}{2^m}\right)
=\left(\sum_k \sqrt{\frac{\alpha_k}{2^m}}\right)^2
\le(\sum_k \alpha_k)\left(\sum_k \frac{1}{2^m}\right)
= \frac{2^n}{2^m}.
\end{align}
Here in the inequality we have used 
Cauchy–Schwarz inequality.
\end{proof}


\subsection{Results}
We show the $O(\log\secp)$ lower bound for the size (i.e., the number of qubits) of the commitment register as follows.
\begin{theorem}\label{thm:lower_bound_SBCH}
There do not exist statistically-binding and computationally-hiding non-interactive quantum bit commitments 
with the $O(\log\secp)$-qubit commitment register.
\end{theorem}

\begin{theorem}\label{thm:lower_bound_SHCB}
There do not exist statistically-hiding and computationally-binding non-interactive quantum bit commitments 
with the $O(\log\secp)$-qubit commitment register.
\end{theorem}

\begin{remark}
Because non-interactive quantum commitments for bit strings    
are those for a single bit,\footnote{Assume that there exists a non-interactive commitment scheme for $n$ bits with some definition of binding. 
Then it is a non-interactive commitment scheme for a single bit with the honest binding of \cref{def:honest_binding}, because
we have only to commit $0^n$ (resp. $1^n$) when we want to commit 0 (resp. $1$),
and any reasonable definition of binding should satisfy the honest binding of \cref{def:honest_binding}. However, it contradicts
\cref{thm:lower_bound_SBCH,thm:lower_bound_SHCB}.} the above theorems also prohibit
non-interactive quantum commitments for bit strings with the $O(\log\secp)$-qubit commitment register.    
Moreover, because commitments for quantum states are also those for a single bit,
above theorems also prohibit non-interactive quantum commitments for quantum states with the $O(\log\secp)$-qubit commitment 
register.
\end{remark}

\begin{remark}
It is known that interactive commitments can be made non-interactive~\cite{AC:Yan22,STOC:GJMZ}, but
that transformation could increase the commitment size. (Honest receiver's register in the interactive commitment scheme
is contained in the commitment register of the non-interactive one.) Therefore 
our no-go results, \cref{thm:lower_bound_SBCH,thm:lower_bound_SHCB}, do not directly exclude 
interactive commitments with the commitment size $O(\log\secp)$.
It is an open problem whether interactive commitments with
the commitment size $O(\log\secp)$ are possible or not.
\end{remark}



These results are tight lower bounds, because we can also show the $\omega(\log\secp)$ upper bounds as follows:
\begin{theorem}\label{thm:upper_bound_SBCH}
If exponentially secure PRGs exist, then
statistically-binding and computationally-hiding non-interactive quantum bit commitments 
with the $m(\secp)$-qubit commitment register exist for any QPT computable function $m(\secp)=\omega(\log\secp)$.
\end{theorem}

\begin{theorem}\label{thm:upper_bound_SHCB}
If exponentially secure PRGs exist, then
statistically-hiding and computationally-binding non-interactive quantum bit commitments 
with the $m(\secp)$-qubit commitment register exist for any QPT computable function $m(\secp)=\omega(\log\secp)$.
\end{theorem}

\if0
\begin{remark}
There are two open problems.
\begin{enumerate}
\item 
Can we weaken the assumption of exponentially secure PRGs to the standard PRGs (or even further weaker ones such as PRSGs or OWSGs)?
\item 
\cref{thm:upper_bound_SBCH,thm:upper_bound_SHCB} show the existence of non-interactive {\it bit} commitments with the $\omega(\log\secp)$-qubit commitment register. 
Can we construct non-interactive quantum commitments where $\poly(\secp)$-bit strings (or even $\poly(\secp)$-qubit quantum states)
can be committed with the $\omega(\log\secp)$-qubit commitment register?\footnote{
Note that it is impossible classically: Let $Com(m,r)$ be the commitment, where $m$ is the message committed and
$r$ is the decommitment. If $|Com(m,r)|$ is much shorter than $|m|$, there is a collision, i.e., $(m,r)$ and $(m',r')$ such that
$Com(m,r)=Com(m',r')$. If such a collision is hardwired in the adversary's algorithm,
the binding is not possible.
%(In the random oracle model,
%there exist statistically-hiding and collapse-binding non-interactive classical commitments
%where $\poly(\secp)$-bit strings can be committed and the size of the commitment is $\omega(\log\secp)$.
%commitments are possible, for example, by using collapsing hash functions~\cite{EC:Unruh16,AC:Unruh16}.
%(\mor{The random oracle can be replaced with collapsing hash functions that can be implemented with several assumptions, such as LWE~\cite{AC:Unruh16}, but in that case
%we need the setup that distributes the key of the hash function.})
For the quantum case, \cite{STOC:GJMZ} constructed non-interactive quantum commitments where $\poly(\secp)$-qubit quantum states
can be committed
with the $\secp$-qubit commitment register, but hiding is not shown.
}
\mor{If there exist collapsing hash functions $H_k:\bit^n\to\bit^m$ with
$n=\poly(\secp)$ and $m=\omega(\log\secp)$,
then $\sum_{k}\ket{k}_\regR\ket{k,H_k(x)}_\regC$ seems to be a statistically-hiding and swap-binding non-interactive
commitments where $\poly(\secp)$-bits are committed with $\omega(\log\secp)$-qubit commitment register.}
\end{enumerate}
\end{remark}
\fi

Because statistically-binding and computationally-hiding non-interactive quantum bit commitments are EFI pairs, 
\cref{thm:lower_bound_SBCH,thm:upper_bound_SBCH} imply the following corollaries.
\begin{corollary}
There do not exist 
$O(\log\secp)$-qubit EFI pairs.
\end{corollary}
\minki{I guess EFI requires only $1/\poly$-far? In that case, the second case of lower bounds for computationally hiding and computationally binding commitment implies this corollary, not \cref{thm:lower_bound_SBCH}?}
\mor{Yes.}

\begin{corollary}
If exponentially secure PRGs exist, then
$m(\secp)$-qubit EFI pairs exist for any QPT computable function $m(\secp)=\omega(\log\secp)$.
\end{corollary}


\subsection{Proofs}

\begin{proof}[Proof of \cref{thm:lower_bound_SBCH}]
Let $(Q_0,Q_1)$ be a statistically-binding and computationally-hiding
non-interactive quantum bit commitment scheme 
with the $m$-qubit commitment register.
Due to the statistical binding, $F(\rho_0,\rho_1)\le\negl(\secp)$ has to be satisfied.\footnote{
The reason is as follows.
If
$F(\rho_0,\rho_1)\ge\frac{1}{p(\secp)}$ for a polynomial $p$ for infinitely many $\secp$, there exists a unitary $V$ such that
$|\langle\Psi_{0}|(V_\regR\otimes I_\regC)|\Psi_{1}\rangle|^2\ge\frac{1}{p(\secp)}$ for infinitely many $\secp$ due to the Uhlmann's theorem.
Then, we have the following unbounded attack to the binding: commit $0$ honestly, apply $V$ on $\regR$, and open the commitment as $1$.}
For each $b\in\bit$, let $\rho_b=\sum_i p_{b,i}|\phi_{b,i}\rangle\langle\phi_{b,i}|$    
be $\rho_b$'s diagonalization.
Then,
\begin{align}
1-\negl(\secp)&\le \|\rho_0-\rho_1\|_{tr}    \\
&=
\left\|\sum_{i}p_{0,i}|\phi_{0,i}\rangle\langle\phi_{0,i}|-\sum_{j}p_{1,j}|\phi_{1,j}\rangle\langle\phi_{1,j}|\right\|_{tr}\\
&=\left\|\sum_{i,j}p_{0,i}p_{1,j}\left(|\phi_{0,i}\rangle\langle\phi_{0,i}|-|\phi_{1,j}\rangle\langle\phi_{1,j}|\right)\right\|_{tr}\\
&\le \sum_{i,j}p_{0,i}p_{1,j}\left\||\phi_{0,i}\rangle\langle\phi_{0,i}|-|\phi_{1,j}\rangle\langle\phi_{1,j}|\right\|_{tr}\\ 
&= \sum_{i,j}p_{0,i}p_{1,j}\sqrt{1-|\langle \phi_{0,i}|\phi_{1,j}\rangle|^2}\\
&\le  \sqrt{1-\sum_{i,j}p_{0,i}p_{1,j}|\langle \phi_{0,i}|\phi_{1,j}\rangle|^2}\\
&\le  \sqrt{1-\frac{1}{4}\sum_{b,b'\in\bit}\sum_{i,j}p_{b,i}p_{b',j}|\langle \phi_{b,i}|\phi_{b',j}\rangle|^2+\negl(\secp)}\label{swaptest}\\
&\le \sqrt{1-2^{-m}+\negl(\secp)},\label{usingwelch} 
\end{align}
which is a contradiction if $m=O(\log\secp)$,
and therefore the theorem is shown.
Here, we have used \cref{cor:Welch} in \cref{usingwelch}.
Moreover, \cref{swaptest} is derived as follows.
First, from the straightforward calculation,
\begin{align}
   \sum_{b,b'\in\bit}\sum_{i,j}p_{b,i}p_{b',j}|\langle\phi_{b,i}|\phi_{b',j}\rangle|^2 
   =\sum_ip_{0,i}^2+\sum_ip_{1,i}^2
   +2\sum_{i,j}p_{0,i}p_{1,j}|\langle\phi_{0,i}|\phi_{1,j}\rangle|^2.\label{swap1}
\end{align}
Second, we have
\begin{align}
\left|\sum_ip_{b,i}^2- \sum_{i,j}p_{0,i}p_{1,j}|\langle\phi_{0,i}|\phi_{1,j}\rangle|^2\right|\le\negl(\secp)    \label{swap2}
\end{align}
for each $b\in\bit$, because otherwise the QPT adversary who does the swap test 
can distinguish $\rho_0$ and $\rho_1$, which breaks the computational hiding. (Consider the following QPT adversary: given $\rho_b$, run the swap test between
it and $\rho_0$. The probability that the adversary accepts is $p_b\coloneqq\frac{1+\Tr(\rho_b\rho_0)}{2}$. Due to the computational
hiding, $|p_0-p_1|\le\negl(\secp)$, which means that
$|\Tr(\rho_0^2)-\Tr(\rho_0\rho_1)|\le\negl(\secp)$.)
By combining \cref{swap1} and \cref{swap2},
we can derive 
\cref{swaptest}.
\end{proof}


\begin{proof}[Proof of \cref{thm:lower_bound_SHCB}]
To show the theorem, assume that
there exists a statistically-hiding and computationally-binding non-interactive quantum bit commitment scheme
$(Q_0,Q_1)$ with the $O(\log\secp)$-qubit commitment register.
Then, due to the flavor conversion (\cref{lem:flavor}), we have
a statistically-binding and computationally-hiding non-interactive quantum bit commitment scheme
$(\tilde{Q}_0,\tilde{Q}_1)$ with $|\regR'|=|\regC|=O(\log\secp)$,
where $|\regA|$ is the number of qubits of the register $\regA$.
However, we can show that such commitments do not exist, because we can construct a QPT adversary that
breaks the hiding as follows:
\begin{enumerate}
    \item 
    Given $\tilde{\rho}_b\coloneqq\Tr_{\regR'}(\ket{\tilde{\Psi}_b}_{\regR',\regC'})$ as input.
    \item 
    Run the swap test between $\tilde{\rho}_0$ and $\tilde{\rho}_b$.
    \item 
    Output the output of the swap test.
\end{enumerate}
Then the probability $p_b$ that the adversary outputs 1 is
   $p_0=\frac{1+\Tr(\tilde{\rho}_0^2)}{2}$ and
   $p_1=\frac{1+\Tr(\tilde{\rho}_0\tilde{\rho}_1)}{2}$. 
Because of the statistical binding, we have $F(\tilde{\rho}_0,\tilde{\rho}_1)\le\negl(\secp)$. Therefore, by using \cref{lem:TrF},
\begin{align}
\Tr(\tilde{\rho}_0\tilde{\rho}_1)\le F(\tilde{\rho}_0,\tilde{\rho}_1)\le\negl(\secp).    
\end{align}
On the other hand, because $|\regR'|=O(\log\secp)$,
\begin{align}
\Tr(\tilde{\rho}_0^2)\ge\frac{1}{\poly(\secp)}.    
\end{align}
Therefore the QPT adversary can break the computational hiding.
\end{proof}


\begin{proof}[Proof of \cref{thm:upper_bound_SBCH}]
Let $G:\bit^\secp\to\bit^{2\secp}$ be an exponentially secure PRG. It means that
there exists a constant $0<c<1$ such that for any QPT adversary $\cA$
\begin{align}
\left|\Pr_{x\gets\bit^\secp}[1\gets\cA(1^\secp,G(x))]    
-\Pr_{y\gets\bit^{2\secp}}[1\gets\cA(1^\secp,y)]    \right|\le 2^{-c\secp}
\end{align}
for all sufficiently large $\secp$.
If we replace $\secp$ with a QPT computable function $n(\secp)= \omega(\log\secp)$, we have
\begin{align}
\left|\Pr_{x\gets\bit^n}[1\gets\cA(1^n,G(x))]    
-\Pr_{y\gets\bit^{2n}}[1\gets\cA(1^n,y)]    \right|\le 2^{-cn}=\negl(\secp)
\end{align}
for sufficiently large $\secp$.
Hence we have a PRG, $G:\bit^n\to\bit^{2n}$.
With this PRG, define the non-interactive quantum bit commitment $(Q_0,Q_1)$ as follows:
\begin{align}
\ket{\Psi_0}_{\regR,\regC}&\coloneqq\frac{1}{\sqrt{2^n}} \sum_{x\in\bit^n}|x0^n\rangle_\regR\otimes |G(x)\rangle_\regC,\label{com1}\\
\ket{\Psi_1}_{\regR,\regC}&\coloneqq\frac{1}{\sqrt{2^{2n}}} \sum_{y\in\bit^{2n}}|y\rangle_\regR\otimes|y\rangle_\regC.\label{com2}
\end{align}
Its computational hiding is clear.
For its statistical binding, from \cref{lem:fidelity_upperbound}, we have
\begin{align}
F(\rho_0,\rho_1)\le 2^{-n}    =\negl(\secp),
\end{align}
which is enough for the sum-binding~\cite{C:MorYam22}.
The number of qubits of the commitment register is $2n=\omega(\log\secp)$.
\end{proof}


\begin{proof}[Proof of \cref{thm:upper_bound_SHCB}]
From the flavor conversion (\cref{lem:flavor}), we can construct
a statistically-hiding and computationally-binding quantum bit commitment scheme from \cref{com1,com2}.
The number of qubits of its commitment register is $|\regC'|=|\regR|+|\regD|=2n+1=\omega(\log\secp)$.
\end{proof}


\subsection{}
\begin{theorem}
There do not exist computationally-binding and computationally-hiding non-interactive quantum bit commitments 
with the $O(\log\secp)$-qubit commitment register.
\end{theorem}

\begin{proof}
Assume that    
such a commitment scheme $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\mathbb{N}}$ exists,
and let $\ket{\Psi_{\secp,b}}_{\regR,\regC}\coloneqq Q_b(\secp)|0...0\rangle$.
Let $\rho^b_{\secp,\regC}\coloneqq \Tr_{\regR}(\ket{\Psi_{\secp,b}}_{\regR,\regC})$.
We consider two cases separately.
\begin{enumerate}
    \item 
$\left\|\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC}\right\|_{tr}\le\negl(\secp)$.
\item 
There exists a polynomial $p$ such that
$\left\|\rho^0_{\secp,\regC}-\rho_{\secp,\regC}^1\right\|_{tr}\ge\frac{1}{p(\secp)}$ for infinitely many $\secp$.
\end{enumerate}
We first consider the case 1.
In that case, $\ket{\Psi_{\secp,b}}$ is actually computationally-binding and statistically-hiding commitment
with $|\regC|=O(\log\secp)$, but it is prohibited from \cref{thm:lower_bound_SHCB}.

\if0
In that case, there exists a polynomial $q$ such that
$\TD(\rho^0_\regR,\rho_\regR^1)\ge\frac{1}{q(\secp)}$ for infinitely $\secp$,
because of the following reason:
If $\TD(\rho^0_\regC,\rho_\regC^1)\le\negl(\secp)$,
then it is actually a computationally-binding and statistically-hiding commitment.
By using \cref{lem:flavor}, we have
a statistically-binding and computationally-hiding commitment 
$\ket{\Psi'_b}_{\regC',\regR'}\coloneqq |0\rangle_\regD|\Psi_0\rangle_{\regC,\regR}+(-1)^b|1\rangle_\regD|\Psi_1\rangle_{\regC,\regR}$ with 
$\regC'\coloneqq(\regR,\regD)$ and $\regR'\coloneqq\regC$,
where $|\regR'|=O(\log\secp)$.
If $\TD(\rho_{\regC'}^0,\rho_{\regC'}^1)\le\negl(\secp)$,
then $F(\rho_{\regC'}^0,\rho_{\regC'}^1)\ge1-\negl(\secp)$.
Then due to the Uhlmann's theorem, there exists a unitary on $\regR'$ such that
$|\langle \Psi'_0|U_{\regR'}\otimes I_{\regC'}|\Psi'_1\rangle|^2\ge1-\negl(\secp)$.
However, it contradicts the fact that $\ket{\Psi'_b}$ is statistically binding.
Hence there exists a polynomial $q$ such that
$\TD(\rho_{\regC'}^0,\rho_{\regC'}^1)\ge\frac{1}{q(\secp)}$ for infinitely many $\secp$.
However, if
$\TD(\rho_{\regC'}^0,\rho_{\regC'}^1)\ge\frac{1}{q(\secp)}$, there exists a QPT attack for the computational hiding of $\ket{\Psi'_b}$ as follows.
Denote $\ket{\Psi'_b}_{\regR',\regC'}=\sum_{i=1}^mc_i|i\rangle_{\regR'}|\phi_i^b\rangle_{\regC'}$, where $m=O(\poly(\secp))$.
Then $\rho_{\regC'}^b=\sum_{i=1}^m|c_i|^2 |\phi_i^b\rangle\langle\phi_i^b|$.
If we define $\Pi\coloneqq \frac{1}{m}\sum_{i=1}^m|\phi_i^b\rangle\langle\phi_i^b|$, we have
$\Tr(\Pi\rho_{\regC'}^1)\le\frac{1}{2q(\secp)}$, because if $\Tr(\Pi\rho_{\regC'}^1)\ge\frac{1}{2q(\secp)}$, 
\begin{align}
\frac{1}{q(\secp)}&\le\Tr(\Pi \rho_{\regC'}^0)
-\Tr(\Pi \rho_{\regC'}^1)\\
&\le     
1-\frac{1}{2q(\secp)}
\end{align}
\fi

Next, consider the case 2.
Let 
$\Pi_\secp\coloneqq\sum_{i=1}^\xi|\eta_{\secp,i}\rangle\langle\eta_{\secp,i}|$, where $\{|\eta_{\secp,i}\rangle\}_{i=1}^\xi$
be the set of all eigenvectors of $\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC}$ corresponding to non-negative eigenvalues.
Then, for each $\secp$ such that
$\left\|\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC}\right\|_{tr}\ge\frac{1}{p(\secp)}$, we have 
\begin{align}
\Tr[\Pi_\secp(\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC})]
=\left\|\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC}\right\|_{tr}\ge\frac{1}{p(\secp)}.
\end{align}

Because $|\regC|=O(\log\secp)$, $\xi=O(\poly(\secp))$.
Moreover, because each $|\eta_{\secp,i}\rangle$ is an $O(\log\secp)$-qubit state,
the unitary $U_{\secp,i}$ such that $U_{\secp,i}|0...0\rangle=|\eta_{\secp,i}\rangle$ can be implemented with a quantum circuit
whose classical description requires only
$O(\poly(\secp))$ bits.\footnote{Any $\log(\secp)$-qubit unitary
can be implemented with a $\poly(\secp)$-depth quantum circuit~\cite{Nielsen_Chuang}.}
\mor{If we use tomography, we can avoid the advice.}
Let us consider the following QPT adversary $\cA$ with classical advice that breaks the computational hiding:
\begin{enumerate}
    \item 
    Get the classical description of $\{U_{\secp,i}\}_{i=1}^\xi$ as advice.
    \item 
    Sample $j\gets [\xi]$.
    \item 
    Apply $U_{\secp,j}$ on the given state $\rho$ (that is $\rho^0_{\secp,\regC}$ or $\rho^1_{\secp,\regC}$), and measure all qubits in the
    computational basis. If all results are 0, output 1.
    Otherwise, output 0.
\end{enumerate}
Then,
\begin{align}
\left|
\Pr[1\gets\cA(\rho^0_{\secp,\regC})]-
\Pr[1\gets\cA(\rho^1_{\secp,\regC})]\right|
&=\frac{1}{\xi}\Tr[\Pi_\secp (\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC})]    \\
&=\frac{1}{\xi}\left\|\rho^0_{\secp,\regC}-\rho^1_{\secp,\regC}\right\|_{tr}    \\
&\ge\frac{1}{\poly(\secp)}
\end{align}
for infinitely many $\secp$. Hence the computational hiding is broken.

\if0
we can get an approximate classical description $[\rho^b_\regC]$ of $\rho_\regC^b$ such that
$\TD(\rho^b_\regC,[\rho^b_\regC])\le\frac{1}{r}$ for any polynomial $r$ 
in a polynomial time (except for a negligible failure probability).
Then, $\TD(\rho^0_\regC-\rho^1_\regC,[\rho^0_\regC]-[\rho^1_\regC])\le\frac{2}{r}$.
Compute $\Pi$ such that $\TD([\rho^0_\regC],[\rho^1_\regC])=\Tr(\Pi(\rho^0_\regC-\rho^1_\regC))$,
which can be done in polynomial time.
\fi
\end{proof}

\if0
\subsection{Swap-Binding Commitments from Collapsing Hash}
\mor{For classical bit strings, $\sum_k\ket{k}_R\ket{H_k(m)}_C$ is stat hiding and collapse binding, and
from exp-secure LWE, $\omega(\log)$-output collapsing $H_k$ can be constructed.
For quantum states, $\sum_k\ket{k}_CU_k\ket{\psi}_R$ is not know to be hiding.
Also, hash-hadamard-hash is not known to be hiding.}
\mor{under const}
Let $h_k:\bit^n\to\bit^m$ be a collapsing hash function with $k\in\bit^\kappa$.
Given the first register of a state $\ket{\psi}=\sum_{x\in\bit^n} c_x |x\rangle|\xi_x\rangle$ as input, the commitment algorithm runs as follows.
\begin{enumerate}
    \item 
    Generate the state 
    \begin{align}
    \left(\frac{1}{\sqrt{2^\kappa}}\sum_{k\in \bit^\kappa}\ket{k}\right)\otimes\left(\sum_xc_x|x\rangle|\xi_x\rangle\right).
    \end{align}
    \item 
    Apply the hash coherently.
    \begin{align}
    \frac{1}{\sqrt{2^\kappa}}\sum_{k,x}c_x|k\rangle|x\rangle|\xi_x\rangle|h_k(x)\rangle.
    \end{align}
    \item 
    Apply the Hadamard on every qubit of the second register.
    \begin{align}
    \frac{1}{\sqrt{2^{\kappa+n}}}\sum_{k,x}\sum_{d\in\bit^n}c_x(-1)^{d\cdot x}|k\rangle|d\rangle|\xi_x\rangle|h_k(x)\rangle.
    \end{align}
    \item 
    Apply the hash coherently.
    \begin{align}
    \frac{1}{\sqrt{2^{\kappa+n}}}\sum_{k,x,d}c_x(-1)^{d\cdot x}|k\rangle|d\rangle|\xi_x\rangle|h_k(x)\rangle|h_k(d)\rangle.
    \end{align}
    \item
    Copy the key of the hash.
    \begin{align}
    \frac{1}{\sqrt{2^{\kappa+n}}}\sum_{k,x,d}c_x(-1)^{d\cdot x}|k\rangle_{\regR_1}|d\rangle_{\regR_2}|\xi_x\rangle_{\regR_3}
    |h_k(x)\rangle_{\regC_1}|h_k(d)\rangle_{\regC_2}|k\rangle_{\regC_3}.
    \end{align}
\end{enumerate}
First, we show the statistical hiding.


Next, we show the swap binding.
First, trace out $\regC_3$. Then we have 
\begin{align}
\frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes|\psi_k\rangle\langle\psi_k|_{\regR_2,\regR_3,\regC_1,\regC_2}, 
\label{ave_k}
\end{align}
where
    \begin{align}
    |\psi_k\rangle\coloneqq\frac{1}{\sqrt{2^n}}\sum_{x,d}c_x(-1)^{d\cdot x}|d\rangle_{\regR_2}|\xi_x\rangle_{\regR_3}
    |h_k(x)\rangle_{\regC_1}|h_k(d)\rangle_{\regC_2}.
    \end{align}
    Let $U^k_{\regR_2,\regC_2}$ be the unitary that applies the Hadamard each qubit of $\regR_2$, and then writes the hash value of
    $\regR_2$ (corresponding to the key $k$) on $\regC_2$. Then 
    \begin{align}
    |\psi_k\rangle= U^k_{\regR_2,\regC_2}
    \sum_{x}c_x|x\rangle_{\regR_2}|\xi_x\rangle_{\regR_3}
    |h_k(x)\rangle_{\regC_1}|0...0\rangle_{\regC_2}.
    \end{align}
    If we trace out $\regC_1$ of \cref{ave_k}, it becomes
\begin{align}
     &\frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes
     U^k_{\regR_2,\regC_2}\sum_y\left(\sum_{x:h_k(x)=y} c_x|x\rangle_{\regR_2}
     |\xi_x\rangle_{\regR_3}|0...0\rangle_{\regC_2}\right)(h.c.) U^{k,\dagger}_{\regR_2,\regC_2}.
    \end{align}
    Due to the collapsing, it is computationally indistinguishable from
    \begin{align}
     &\frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes
     U^k_{\regR_2,\regC_2}\left(\sum_x |c_x|^2|x\rangle\langle x|_{\regR_2}
     \otimes |\xi_x\rangle\langle \xi_x|_{\regR_3}\otimes |0...0\rangle\langle0...0|_{\regC_2}\right) U^{k,\dagger}_{\regR_2,\regC_2}\\
     &=
     \frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes
     \sum_x 
     |c_x|^2
     |\xi_x\rangle\langle \xi_x|_{\regR_3}
     \otimes\left[\frac{1}{\sqrt{2^n}}\sum_d(-1)^{d\cdot x}|d\rangle_{\regR_2}|h_k(d)\rangle_{\regC_2}\right]
     \left[h.c.\right].
    \end{align}
   If we trace out $\regC_2$, it becomes
   \begin{align}
     \frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes
     \sum_x 
     |c_x|^2
     |\xi_x\rangle\langle \xi_x|_{\regR_3}
     \otimes\sum_e
     \left[\frac{1}{\sqrt{2^n}}\sum_{d:h_k(d)=e}(-1)^{d\cdot x}|d\rangle_{\regR_2}\right]
     \left[h.c.\right].
    \end{align}
   Due to the collapsing, it is computationally indistinguishable from
    \begin{align}
     & \frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes
     \sum_x 
     |c_x|^2
     |\xi_x\rangle\langle \xi_x|_{\regR_3}\otimes
     \frac{1}{2^n}\sum_d|d\rangle\langle d|_{\regR_2}\\
     &=\left(\frac{I^{\otimes \kappa}}{2^\kappa}\right)_{\regR_1}
     \otimes
      \sum_x 
     |c_x|^2
     |\xi_x\rangle\langle \xi_x|_{\regR_3}\otimes
     \left(\frac{I^{\otimes n}}{2^n}\right)_{\regR_2}.
    \end{align}
    \fi
    
    
\if0
    If we measure $\regC_2$ in the computational basis, the state becomes
    \begin{align}
\frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes\sum_e  |\psi_{k,e}\rangle\langle\psi_{k,e}|_{\regR_2,\regR_3,\regC_1}, \label{collapse1}
    \end{align}
    where
    \begin{align}
    \ket{\psi_{k,e}}&\coloneqq
    \frac{1}{\sqrt{2^n}}\sum_{x}\sum_{d:h_k(d)=e}c_x(-1)^{d\cdot x}|d\rangle_{\regR_2}|\xi_x\rangle_{\regR_3}
    |h_k(x)\rangle_{\regC_1}\\
    &=
   \frac{1}{\sqrt{2^n}}\sum_{d:h_k(d)=e}\left[\sum_xc_x(-1)^{d\cdot x}|\xi_x\rangle_{\regR_3}|h_k(x)\rangle_{\regC_1}\right]|d\rangle_{\regR_2}\\
   &\coloneqq
   \frac{1}{\sqrt{2^n}}\sum_{d:h_k(d)=e}|\eta_{k,d}\rangle_{\regR_3,\regC_1}|d\rangle_{\regR_2}.
    \end{align}
    Because of the collapsing, \cref{collapse1} is computationally indistinguishable from
     \begin{align}
\frac{1}{2^\kappa}\sum_k |k\rangle\langle k|_{\regR_1}\otimes\sum_e 
 (\rho_{k,e})_{\regR_2,\regR_3,\regC_1} 
 =
\frac{1}{2^{\kappa+n}}\sum_{k,d} |k\rangle\langle k|_{\regR_1}\otimes
|d\rangle\langle d|_{\regR_2}\otimes
|\eta_{k,d}\rangle\langle\eta_{k,d}|_{\regR_3,\regC_1},
    \end{align}
   where 
    \begin{align}
   \rho_{k,e}\coloneqq\frac{1}{2^n}\sum_{d:h_k(d)=e}
   |\eta_{k,d}\rangle\langle\eta_{k,d}|_{\regR_3,\regC_1}
   \otimes|d\rangle\langle d|_{\regR_2}.
    \end{align}
    \fi
    
 

==> working_log_owsg.tex <==
\section{OWSGs from PRSGs}
\begin{definition}[Pseudo-random quantum states generators (PRSGs)]
    For a function $\epsilon:\mathbb N \to [0,1]$,
    An $\epsilon$-pseudorandom quantum states generator ($\epsilon$-PRSG) is a tuple of QPT algorithms $(\KeyGen,\StateGen)$ that work as follows:
    \begin{itemize}
        \item $\KeyGen(1^\lambda)\to k:$ It is a QPT algorithm that, on input the security parameter $\lambda$, 
        outputs a classical key $k\in\bit^n$.
        \item $\StateGen(k)\to \ket{\phi_k}:$ It is a QPT algorithm that, on input $k$, outputs an $m$-qubit quantum state $\ket{\phi_k}$.
    \end{itemize}
    We require the following pseudorandomness: For any polynomial $t$ and any QPT algorithm $\cA$,
    \[
    \left| 
        \Pr_{k \gets \KeyGen(1^\lambda)} \left[ 
            1 \gets \cA\left(1^\lambda,
                \ket{\phi_k}^{\otimes t}
            \right)
        \right]
        -
        \Pr_{\ket{\psi}\gets \mu_m} \left[ 
            1 \gets \cA\left(1^\lambda,
                \ket{\psi}^{\otimes t}
            \right)
        \right]
    \right|
    \le \epsilon(\lambda)
    \]
    for all sufficiently large $\secp$, where $\mu_m$ is the Haar measure on $m$-qubit quantum states.
    We say that it is a PRSG if it is a $\lambda^{-c}$-PRSG for all $c\in \mathbb N$.
\end{definition}

We recall the following lemma from~\cite[Lemma 3.2]{CGGHLP23} with a small modification.
% \footnote{We only use a slightly better concentration inequality than~\cite[Lemma 3.1]{CGGHLP23}, which says that
%         $\Pr_{\ket{\psi} \gets \mu_m} [ 
%             |\braket{\psi|\phi_0}|^2 \ge h 
%         ] = (1-h)^{2^m-1}$ for any $h\in[0,1]$. The proof of this inequality can be found in the proof of~\cite[Lemma 3.6]{AK07}. Since it is cleaner and better, we choose this bound.} 
        \takashi{I think it's better to write it as a proof sketch rather than just a footnote.}
\begin{lemma}\label{lem:PRSGtoOWSG}
    Let $(\KeyGen,\StateGen)$ be an $\epsilon$-PRSG, where $\StateGen$ maps $n$-bit strings to $m$-qubit pure states. 
    Let $h \in [0,1]$ and $\delta= 2^n \cdot \left(1-h\right)^{2^m-1} + h$.
    Define a QPT algorithm $\Ver(k',\ket{\phi_k}) \to \top/\bot$ to be the projection of $\ket{\phi_k}$ onto $\ket{\phi_{k'}}$ with the output $\top$ only when the projection is successful. 
    Then $(\KeyGen,\StateGen,\Ver)$ is an $(\epsilon+\delta)$-OWSG.
\end{lemma}
\begin{proof}[Proof sketch]
    Most parts of the proof are identical to the original one.
    When proving the security, we recall the following concentration inequality for Haar random states instead of~\cite[Lemma 3.1]{CGGHLP23}. 
    \begin{lemma}\label{lem:Haar_concentration}
        For any $h \in [0,1]$ and for any $m$-qubit quantum state $\phi_0$, it holds that for the Haar measure on $m$-qubit quantum states $\mu_m$,
        \[
            \Pr_{\ket{\psi} \gets \mu_m} \left[ 
                |\braket{\psi|\phi_0}|^2 \ge h 
            \right] 
            = (1-h)^{2^m-1}.
        \]
    \end{lemma}
    The proof of this lemma can be found in the proof of~\cite[Lemma 3.6]{AK07}. Using this inequality instead of~\cite[Lemma 3.1]{CGGHLP23} gives the choice $\delta=2^n \cdot (1-h)^{2^m-1}+h$, where $h$ has a similar role to $1/f(n)$ in the original proof.
    % More precisely, we assume that there exists a QPT adversary $\cA$ that breaks the $(\epsilon+\delta)$-OWSG security of $(\KeyGen,\StateGen,\Ver)$ using $t$ copies of the target state. We construct a new QPT adversary $\cB(1^\lambda,\ket{\phi_k}^{\otimes (t+1)})$ for the $\epsilon$-PRSG $(\KeyGen,\StateGen)$ as follows.
    % \begin{enumerate}
    %     \item Run $k' \gets \cA(1^\lambda,\ket{\psi}^{\otimes t})$ for the $t$ copies.
    %     \item Run $\top/\bot \gets \Ver(k',\ket{\psi})$ using the last copy.
    %     \item Output $1$ if the answer of $\Ver$ is $\top$, else output $0$.
    % \end{enumerate}
    %
    % If $\ket{\psi} = \ket{\phi_k}$ for some $k\gets\KeyGen(1^\lambda)$, the probability that $\cB$ outputs $1$ is computed by
    % \begin{align}
    %     &\Pr_{k \gets \KeyGen(1^\lambda)} \left[
    %         1\gets \cB\left(1^\lambda,\ket{\phi_k}^{\otimes (t+1)}\right) 
    %     \right]\\
    %     &=
    %     \Pr \left[
    %         \top \gets \Ver(k',\ket{\phi_k}) : k\gets \KeyGen(1^\lambda),k' \gets \cA(1^\lambda,\ket{\psi}^{\otimes t})
    %     \right] \ge \epsilon+\delta.
    % \end{align}
    %
    % On the other hand, if the target state is Haar random, we have
    % \begin{align}
    %     \Pr_{\ket{\psi}\gets \mu_m} \left[
    %         1\gets \cB\left(1^\lambda,\ket{\psi}^{\otimes (t+1)}\right) 
    %     \right]
    %     &=
    %     \mathbb{E}_{\ket{\psi}\gets \mu_m} \left[
    %         |\braket{\psi|\phi_k}|^2 \left |
    %         k\gets \cA(1^\lambda,\ket{\psi}^{\otimes t})
    %     \right.
    %     \right]
    %     \\&\le\label{eqn:PRSG=>OWSG_exp_max}
    %     \mathbb{E}_{\ket{\psi}\gets \mu_m} \left[
    %         \max_{k \in \bit^n} |\braket{\psi|\phi_k}|^2
    %     \right].
    % \end{align}
    % Here we use~\Cref{lem:Haar_concentration}. By the union bound, it holds that for any $h\in [0,1]$
    % \begin{align}
    %     \Pr_{\ket{\psi} \gets \mu_m} \left[ 
    %         \max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h 
    %     \right] 
    %     \le 2^n (1-h)^{2^m-1}.
    % \end{align}
    % By dividing two cases based on $\max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h $ or not, \Cref{eqn:PRSG=>OWSG_exp_max} is bounded above by
    % \begin{align}
    %     \Pr_{\ket{\psi} \gets \mu_m} \left[ 
    %         \max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h 
    %     \right] + h \le 2^n (1-h)^{2^m-1} + h = \delta.
    % \end{align}
    % This completes the proof.
\end{proof}

\begin{theorem}
    Let $c\in \mathbb{N}$. If there exist OWFs, then there exist $\lambda^{-c}$-OWSGs with $m(\lambda)$-qubit pure state outputs for some 
    $m(\secp)=(c+1) \log \lambda+O(1).$
\end{theorem}
% \minki{Is there any better expression for $m$? I think the lower bound from the Welch bound gives $m= \Omega(c\log \lambda)$ in a similar setting.}
% \takashi{I think $(c+1)\log \lambda +O(1)$ suffices as seen as follows: there is a constant $K$ such that for $\lambda\ge K$,  
% $2^{\lambda+2}\lambda^c\le e^{\lambda}$.  
% This means that $2^{\lambda+2}\lambda^c\le 
%  e^{\lambda}+\max_{\lambda\in[K]}(2^{\lambda+2}\lambda^c-e^{\lambda})=
% e^{\lambda}+O(1)$. 
% I believe this gives $m=(c+1)\log \lambda +O(1)$
% (Actually, I guess the constant additive term can be $2$ or $3$ if we calculate more carefully, but I don't think that's needed)
% }
\begin{proof}
    By~\cite{C:BraShm20}, there exist PRSGs with input length $\lambda$ and any output length $m$ assuming the existence of OWFs.
    We apply~\Cref{lem:PRSGtoOWSG} with $h=\lambda^{-c}/4$ and
    \begin{align}
        m\ge 
        \log \left(
            \frac{\log_e\left(
                2^{\lambda+2}\lambda^c
            \right)}{h}+1
        \right)~\Longrightarrow~2^n \cdot (1-h)^{2^m-1} \le \lambda^{-c}/4,
    \end{align}
    which gives $\delta=\lambda^{-c}/2$.
    To prove the asymptotic bound of $m(\lambda)$, we choose a constant $K$ such that $2^{\lambda+2}\lambda^c \le e^\lambda$ for all $\lambda\ge K$. In this case, the minimal $m$ satisfies
    \begin{align}
        m \ge \log \left(
            4 \lambda^{c+1} + 1
        \right)
        \ge (c+1) \log \lambda + 3,
    \end{align}
    thus we can choose $m(\lambda)=(c+1)\log \lambda +O(1)$.
\end{proof}
\begin{remark}
    (Some discussion about the gap between the lower bound of $m \ge c\log\lambda$ necessary from the Welch bound \takashi{I guess this bound is only for pure case. For the mixed case, the bound will be slightly different. We may need to write it later.}
    and $m \ge (c+1)\log \lambda +o(c\log \lambda)$ upper bound. Also the above construction does not give log-log length OWSGs for $c=0$) \takashi{I know what you want to mean here, but the case of $c=0$ does not make sense in this context since $\lambda^{-0}=1$ and $1$-OWSG can have $0$-qubit outputs.}
\end{remark}






\minki{I notice that the below are very small improvements over~\cite[Lemma 3.2]{CGGHLP23}, thus just citing it instead and mentioning how to improve..}
% We first recall the following concentration inequality for Haar random states, which can be found in the proof of~\cite[Lemma 3.6]{AK07}.
% \begin{lemma}\label{lem:Haar_concentration}
%     For any $h \in [0,1]$ and for any $m$-qubit quantum state $\phi_0$, it holds that for the Haar measure on $m$-qubit quantum states $\mu_m$,
%     \[
%         \Pr_{\ket{\psi} \gets \mu_m} \left[ 
%             |\braket{\psi|\phi_0}|^2 \ge h 
%         \right] 
%         = (1-h)^{2^m-1}.
%     \]
% \end{lemma}
% The following lemma is a variant of~\cite[Lemma 3.2]{CGGHLP23} with some parameter adjustments.
% \begin{lemma}
    % Let $(\KeyGen,\StateGen)$ is a $\epsilon$-PRSG taking $n$-bit strings to $m$-qubit pure states. Define a QPT algorithm $\Ver(k',\ket{\psi_k}) \to \top/\bot$ to be the projection of $\ket{\phi_k}$ onto $\ket{\phi_{k'}}$ with the output $\top$ only when the projection is successful. Then $(\KeyGen,\StateGen,\Ver)$ is ...OWSG.
% \end{lemma}
% \begin{proof}
%     The correctness of $\Ver$ is obvious, and it suffices to argue the security.
%     Toward contradiction, we assume that there exists a QPT adversary $\cA$ that breaks the $(\epsilon+\delta)$-OWSG security of $(\KeyGen,\StateGen,\Ver)$ using $t$ copies of the target state. We will construct a new QPT adversary $\cB(1^\lambda,\ket{\phi_k}^{\otimes (t+1)})$ for the $\epsilon$-PRSG $(\KeyGen,\StateGen)$ as follows.
%     \begin{enumerate}
%         \item Run $k' \gets \cA(1^\lambda,\ket{\psi}^{\otimes t})$ for the $t$ copies.
%         \item Run $\top/\bot \gets \Ver(k',\ket{\psi})$ using the last copy.
%         \item Output $1$ if the answer of $\Ver$ is $\top$, else output $0$.
%     \end{enumerate}
    
%     If $\ket{\psi} = \ket{\phi_k}$ for some $k\gets\KeyGen(1^\lambda)$, the probability that $\cB$ outputs $1$ is computed by
%     \begin{align}
%         &\Pr_{k \gets \KeyGen(1^\lambda)} \left[
%             1\gets \cB\left(1^\lambda,\ket{\phi_k}^{\otimes (t+1)}\right) 
%         \right]\\
%         &=
%         \Pr \left[
%             \top \gets \Ver(k',\ket{\phi_k}) : k\gets \KeyGen(1^\lambda),k' \gets \cA(1^\lambda,\ket{\psi}^{\otimes t})
%         \right] \ge \epsilon+\delta.
%     \end{align}
%     where the last inequality is due to the assumption that $\cA$ breaks $(\epsilon+\delta)$-OWSG security.

%     On the other hand, if the target state is Haar random, we have
%     \begin{align}
%         \Pr_{\ket{\psi}\gets \mu_m} \left[
%             1\gets \cB\left(1^\lambda,\ket{\psi}^{\otimes (t+1)}\right) 
%         \right]
%         &=
%         \mathbb{E}_{\ket{\psi}\gets \mu_m} \left[
%             |\braket{\psi|\phi_k}|^2 \left |
%             k\gets \cA(1^\lambda,\ket{\psi}^{\otimes t})
%         \right.
%         \right]
%         \\&\le\label{eqn:PRSG=>OWSG_exp_max}
%         \mathbb{E}_{\ket{\psi}\gets \mu_m} \left[
%             \max_{k \in \bit^n} |\braket{\psi|\phi_k}|^2
%         \right].
%     \end{align}
%     Here we recall~\Cref{lem:Haar_concentration}: By the union bound, it holds that for any $h\in [0,1]$
%     \begin{align}
%         \Pr_{\ket{\psi} \gets \mu_m} \left[ 
%             \max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h 
%         \right] 
%         \le 2^n (1-h)^{2^m-1}.
%     \end{align}
%     By dividing two cases based on $\max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h $ or not, \Cref{eqn:PRSG=>OWSG_exp_max} is bounded above by
%     \begin{align}
%         \Pr_{\ket{\psi} \gets \mu_m} \left[ 
%             \max_{k \in \bit^n}|\braket{\psi|\phi_j}|^2 \ge h 
%         \right] + h \le 2^n (1-h)^{2^m-1} + h.
%     \end{align}
% \end{proof}
